FedCluster: Boosting the Convergence of Federated Learning via Cluster-Cycling

We develop FedCluster--a novel federated learning framework with improved optimization efficiency, and investigate its theoretical convergence properties. The FedCluster groups the devices into multiple clusters that perform federated learning cyclically in each learning round. Therefore, each learning round of FedCluster consists of multiple cycles of meta-update that boost the overall convergence. In nonconvex optimization, we show that FedCluster with the devices implementing the local {stochastic gradient descent (SGD)} algorithm achieves a faster convergence rate than the conventional {federated averaging (FedAvg)} algorithm in the presence of device-level data heterogeneity. We conduct experiments on deep learning applications and demonstrate that FedCluster converges significantly faster than the conventional federated learning under diverse levels of device-level data heterogeneity for a variety of local optimizers.

==> RelatedWork.tex <==
\section{Introduction}
<Federated Learning for Resource-Constrained IoT Devices: Panoramas and State-of-the-art>: Fed

\cite{konevcny2016federated} Setting of federated learning

$K$ devices.\\

Provided by recent paper <Federated Continual Learning with Adaptive Parameter Communication> \\
(not sure whether to cite this paper right above)
Typical paper on FedAvg \cite{mcmahan2016communication} and FedProx \cite{li2018federated},


\cite{li2019communication}: $L$-smooth, global SG, local SG variance bounded ($\mathbb{E}_{\xi \sim \mathcal{D}_{k}}\left\|\nabla F_{k}(\boldsymbol{x} ; \xi)-\nabla f_{k}(\boldsymbol{x})\right\|^{2} \leq \sigma^{2}, \quad \forall \boldsymbol{x} \in \mathbb{R}^{d}$), global SG variance bounded ($\frac{1}{n} \sum_{k=1}^{n}\left\|\nabla f_{k}(\boldsymbol{x})-\nabla f(\boldsymbol{x})\right\|^{2} \leq \kappa^{2}, \quad \forall \boldsymbol{x} \in \mathbb{R}^{d}$ non-iid degree bounded)\\

$I_1=E, I_2=1$

$\frac{1}{T} \sum_{t=1}^{T} \mathbb{E}\left\|\nabla f\left(\bar{x}_{t}\right)\right\|^{2}\le\mathcal{O}(\sqrt{\frac{E}{KT}}+\frac{C_1 KE}{T})$. (May be better than us in the non-convex case!) (Ziyi found in FedAvg when $\rho=0$, the error bound becomes $\mathcal{O}(\sqrt{\frac{L\sigma^2[f(\overline{x}_0)-f(x^*)]}{KT}})$)


~\\
~\\
~\\
\cite{li2019convergence}: Fed-avg; \\
L-smooth, $\mu$-strongly convex, unbiased stochastic gradient, bounded L2-norm ($G^2$) of stochastic gradient; 
$$\mathbb{E}[F(w_t)-F^*]\le\mathcal{O}\left[\frac{1}{\mu t}\left(L\Gamma+E^2G^2+2L\|w_0-w^*\|\right)\right].$$


\cite{haddadpour2019local}: Fed-avg; \\
unbiased stochastic gradient, bounded stochastic variance on the \textbf{whole} data (); $L$-smoothness, $\mu$-Polyak-Lojasiewicz (PL). 
\begin{align*}
	\mathbb{E}[F(w_t)-F^*]\le\mathcal{O}\left(\frac{1}{KBt}\right),
\end{align*}
\noindent where $B$ is local batchsize.\\

\cite{liang2019variance}: FedAvg with shrinkage towards device-average and constant stepsize; $L$-smoothness, nonconvex, SG has no biase and bounded variance. Average gradient norm square $\le\mathcal{O}(1/t+1/K+E)$.


\cite{hanzely2020federated}: Another objective function that allows different parameters among the devices.


Federated learning with matched averaging: The output of many Neural networks does not change with permutation of some parameters. (perhaps unrelated and not needed to mention in introduction)

\cite{ramazanli2020adaptive}: It also aims at solving the heterogenity issue among the devices. However, the SVRG contained in it needs to compute the full gradient periodically, which is computationally heavy in federated setting with a huge number of devices. 

\cite{haddadpour2019convergence}: FedAvg

Federated Visual Classification with Real-World Data Distribution: This paper works on heterogeneity of FedAvg for visual classification, without proof. (Not sure whether to include it yet)


Adaptive Federated Optimization: ``Due to the heterogeneity of the client datasets, standard federated optimization methods such as Federated Averaging (FEDAVG) are often difficult to tune and exhibit unfavorable convergence behavior. In non-federated settings, adaptive optimization methods have had notable success in combating such issues.''; ``we propose federated versions of adaptive optimizers, including ADAGRAD, ADAM, and YOGI''; in nonconvex setting

$E$  


\subsection{Related work}
\cite{dinh2019federated} deals with the heterogeneity problem by improving the objective function for local update. \\

The following papers aims at training local device models as well as the global model with the challenge of data heterogeneity among devices: <<Adaptive Personalized Federated Learning>>, <<Survey of Personalization Techniques for Federated Learning>>, <<Federated Learning of a Mixture of Global and Local Models>>. \\



==> lemma_nc.tex <==
\section{Supporting Lemmas for \Cref{thm: nc}}





==> lemma_sc.tex <==


%\begin{lemma}\label{lemma_fromstar}
%Let \Cref{assum: P} hold. Then, it holds that
%	\begin{align}\label{fromstar}
%	&\mathbb{E} \Big[ f(W^{*}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})})-f(\overline{w}_{j,K,t}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})})\Big]\nonumber\\ 
%	&\le \eta_{j,0,0}EMG^2,
%	\end{align}
%	{where $W^*=\mathop{\arg\min}_{w\in\mathbb{R}^d} f(w)$.}
%\end{lemma}
%
%\begin{proof}
%	Note that $W^*$ and $W_{jM}$ are independent from $\sigma_{j}(K+1)$. We obtain that
%	\begin{align}
%	&\mathbb{E}f(W^{*}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})})=f(W^{*})\nonumber\\
%	&\le \mathbb{E}f(W_{jM})=\mathbb{E}f(W_{jM}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}).\nonumber
%	\end{align}
%	Hence, we further obtain that
%	\begin{align}
%	&\mathbb{E} \Big[ f(W^{*}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})})-f(\overline{w}_{j,K,t}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})})\Big] \nonumber\\
%	&\le\mathbb{E} [f(W_{jM}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})})-f(\overline{w}_{j,K,t}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})})]\nonumber\\
%	&\stackrel{(i)}{\le} G\mathbb{E}\|\overline{w}_{j,K,t}-W_{jM}\|\nonumber\\
%	&\le G\sqrt{\mathbb{E}\|\overline{w}_{j,K,t}-W_{jM}\|^2}\nonumber\\
%	&\stackrel{(ii)}{\le} \eta_{j,0,0}EMG^2,
%	\end{align}
%	\noindent {where (i) uses \eqref{fS_G} and $W_{jM}=\overline{w}_{j,0,0}$ and (ii) uses \Cref{lemma_FedAvg_howfar_strongconvex}. }
%\end{proof}


==> proof_nc.tex <==





==> proof_sc.tex <==
\subsection{Proof of \Cref{thm: sc}}
The proof logic follows that for proving Theorem 1 in \cite{li2019convergence}. However, our proof requires substantial development to address the following two major issues: 1) each learning round of FedCluster consists of $M$ inner cycles, with each cycle corresponding to a FedAvg process performed by a certain cluster; 2) the reshuffled cyclic order indexes $\sigma_j(K+1), K=0,...,M-1$ for the clusters are {\em dependent} on each other.

%The $l_2$ distance of the averaged $\overline{w}_{j,K,t+1}$ to the optimal point $W^*$ can be decomposed as follows
By \eqref{w_avg_update}, we obtain that
\begin{align}\label{werr_decomp}
&\|\overline{w}_{j,K,t+1}-W^*\|^2\nonumber\\
&=\underbrace {\|\overline{w}_{j,K,t}-W^*- \eta_{j,K,t} \overline{g}_{j,K,t}\|^2}_{A_1} +\eta_{j,K,t}^2 \|\overline{g}_{j,K,t}-g_{j,K,t}\|^2 \nonumber\\
&\quad +\underbrace{2\eta_{j,K,t}\langle\overline{w}_{j,K,t}-W^*- \eta_{j,K,t} \overline{g}_{j,K,t}, \overline{g}_{j,K,t}-g_{j,K,t}\rangle}_{A_2}.
\end{align}
Since $\mathbb{E} A_2=0$ by \eqref{Eg}, we next derive an upper bound for $A_1$. We obtain that
\begin{align}\label{A1_decomp}
A_1&=\|\overline{w}_{j,K,t}-W^*-\eta_{j,K,t} \overline{g}_{j,K,t}\|^2\nonumber\\
&=\|\overline{w}_{j,K,t}-W^*\|^2 \underbrace{-2\eta_{j,K,t}\langle \overline{w}_{j,K,t}-W^*, \overline{g}_{j,K,t} \rangle}_ {B_1}\nonumber\\
&\quad +\underbrace{\eta_{j,K,t}^2\|\overline{g}_{j,K,t}\|^2}_{B_2}.
\end{align}
The terms $B_1$ and $B_2$ can be respectively decomposed as follows
\begin{align}\label{B1_decomp}
B_1&=-2\eta_{j,K,t}\langle \overline{w}_{j,K,t}-W^*, \overline{g}_{j,K,t} \rangle\nonumber\\
&=-2\eta_{j,K,t} \sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} \nonumber\\
&\quad\langle \overline{w}_{j,K,t}-W^*, \nabla f(w_{j,K,t}^{(k)}; \mathcal{D}^{(k)})\rangle \nonumber\\
&=-2\eta_{j,K,t} \sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} \nonumber\\
&\quad\langle \overline{w}_{j,K,t}-w_{j,K,t}^{(k)}, \nabla f(w_{j,K,t}^{(k)}; \mathcal{D}^{(k)})\rangle \nonumber\\
&\quad-2\eta_{j,K,t} \sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} \nonumber\\
&\quad\langle w_{j,K,t}^{(k)}-W^*, \nabla f(w_{j,K,t}^{(k)}; \mathcal{D}^{(k)})\rangle \nonumber\\
&\stackrel{(i)}{\le} 2\eta_{j,K,t} \sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}}\Big[ f(w_{j,K,t}^{(k)}; \mathcal{D}^{(k)}) \nonumber\\ 
&\quad- f(\overline{w}_{j,K,t}; \mathcal{D}^{(k)}) +  \frac{L}{2}\|\overline{w}_{j,K,t}-w_{j,K,t}^{(k)}\|^2  \Big]\nonumber\\
&\quad-2\eta_{j,K,t} \sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} \Big[ f(w_{j,K,t}^{(k)}; \mathcal{D}^{(k)})\nonumber\\
&\quad-f(W^*; \mathcal{D}^{(k)}) +\frac{\mu}{2} \|{w_{j,K,t}^{(k)}}-W^*\|^2 \Big]\nonumber\\
&\stackrel{(ii)}{\le} 2\eta_{j,K,t} \Big[ f(W^*; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) - f(\overline{w}_{j,K,t}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) \Big]\nonumber\\
&\quad+L\eta_{j,K,t} \sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} \|\overline{w}_{j,K,t}-w_{j,K,t}^{(k)}\|^2\nonumber\\&\quad -\mu\eta_{j,K,t} \|\overline{w}_{j,K,t}-W^*\|^2
\end{align}
where (i) uses the $L$-smoothness and $\mu$-strong convexity of $f(\cdot; \mathcal{D}^{(k)})$, and (ii) uses $f(w; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})})=\sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} f(w; \mathcal{D}^{(k)})$ and {applies Jensen's inequality to $\|\cdot\|^2$}.
\begin{align}\label{B2_strongconvex}
B_2=&\eta_{j,K,t}^2\|\overline{g}_{j,K,t}\|^2\nonumber\\
=&\eta_{j,K,t}^2\Big\| \sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} \nabla f(w_{j,K,t}^{(k)}; \mathcal{D}^{(k)})\Big\|^2 \nonumber\\
\stackrel{(i)}{\le}& 2\eta_{j,K,t}^2 \Big\|\sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} [\nabla f(w_{j,K,t}^{(k)}; \mathcal{D}^{(k)})\nonumber\\
&-\nabla f(\overline{w}_{j,K,t}; \mathcal{D}^{(k)})] \Big\|^2 \nonumber\\
&+2\eta_{j,K,t}^2 \Big\| [\nabla f(\overline{w}_{j,K,t}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})})] \Big\|^2\nonumber\\
\stackrel{(ii)}{\le}& 2\eta_{j,K,t}^2 \sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} \nonumber\\
&\Big\| \nabla f(w_{j,K,t}^{(k)}; \mathcal{D}^{(k)})-\nabla f(\overline{w}_{j,K,t}; \mathcal{D}^{(k)}) \Big\|^2 \nonumber\\
&+2\eta_{j,K,t}^2 \Big\| \nabla f(\overline{w}_{j,K,t}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) \Big\|^2\nonumber\\
\stackrel{(iii)}{\le}& 2L^2\eta_{j,K,t}^2 \sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}}  \Big\|w_{j,K,t}^{(k)} - \overline{w}_{j,K,t}\Big\|^2 \nonumber\\
&+4L \eta_{j,K,t}^2 \Big[ f(\overline{w}_{j,K,t}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) - f^*(\cdot;\mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) \Big]
\end{align} 
where (i) uses the inequality that $\|a+b\|^2\le 2\|a\|^2+2\|b\|^2$, (ii) applies Jensen's inequality to $\|\cdot\|^2$, and (iii) uses the $L$-smoothness of $f(\cdot; \mathcal{D}^{(k)})$ and $f(\cdot; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})})$. Substituting \eqref{B2_strongconvex} and \eqref{B1_decomp} into \eqref{A1_decomp} yields that
\begin{align}\label{A1_strongconvex}
A_1=&\|\overline{w}_{j,K,t}-W^*\|^2+B_1+B_2 \nonumber\\
\le& \|\overline{w}_{j,K,t}-W^*\|^2\nonumber\\
&+2\eta_{j,K,t} \Big[ f(W^*; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) - f(\overline{w}_{j,K,t}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) \Big]\nonumber\\
&+L\eta_{j,K,t}(1+2L\eta_{j,K,t}) \nonumber\\
&\sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} \|\overline{w}_{j,K,t}-w_{j,K,t}^{(k)}\|^2 \nonumber\\
&-\mu\eta_{j,K,t} \|\overline{w}_{j,K,t}-W^*\|^2 \nonumber\\
&+4L \eta_{j,K,t}^2 \Big[ f(\overline{w}_{j,K,t}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) - f^*(\cdot;\mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) \Big]\nonumber\\
=&2\eta_{j,K,t}(1-2L\eta_{j,K,t})\nonumber\\ 
&\Big[ f(W^*; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) - f(\overline{w}_{j,K,t}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) \Big] \nonumber\\
&+L\eta_{j,K,t}(1+2L\eta_{j,K,t}) \nonumber\\
&\sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} \|\overline{w}_{j,K,t}-w_{j,K,t}^{(k)}\|^2 \nonumber\\
&+4L \eta_{j,K,t}^2 \Big[ f(W^*; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) - f^*(\cdot;\mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) \Big] \nonumber\\
&+(1-\mu\eta_{j,K,t}) \|\overline{w}_{j,K,t}-W^*\|^2 \end{align}

Substituting \eqref{A1_strongconvex} into \eqref{werr_decomp}, taking expectation on both sides and noting that $\mathbb{E} A_2=0$, we obtain that
\begin{align}
&\mathbb{E}\|\overline{w}_{j,K,t+1} - W^*\|^2\nonumber\\
&\le 2\eta_{j,K,t}(1-2L\eta_{j,K,t})\nonumber\\ &\quad\mathbb{E}\Big[ f(W^*; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) - f(\overline{w}_{j,K,t}; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) \Big]\nonumber\\
&\quad+L\eta_{j,K,t}(1+2L\eta_{j,K,t}) \nonumber\\
&\quad\mathbb{E} \Big[\sum_{k\in \mathcal{S}_{\sigma_{j}(K+1)}} \frac{p_k}{q_{\sigma_{j}(K+1)}} \|\overline{w}_{j,K,t}-w_{j,K,t}^{(k)}\|^2\Big] \nonumber\\
&\quad+(1-\mu\eta_{j,K,t}) \mathbb{E}\|\overline{w}_{j,K,t}-W^*\|^2\nonumber\\
&\quad+4L \eta_{j,K,t}^2 \mathbb{E}\Big[ f(W^*; \mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) - f^*(\cdot;\mathcal{D}^{(\mathcal{S}_{\sigma_{j}(K+1)})}) \Big] \nonumber\\
&\quad+\eta_{j,K,t}^2\mathbb{E} \|\overline{g}_{j,K,t}-g_{j,K,t}\|^2\nonumber\\
&\stackrel{(i)}{\le} (1-\mu\eta_{j,K,t}) \mathbb{E}\|\overline{w}_{j,K,t}-W^*\|^2 + 2\eta_{j,K,t}\eta_{j,0,0}EMG^2 \nonumber\\
&\quad+ L\eta_{j,K,t}[1+2L/(4L)]\eta_{j,K,0}^2E^2G^2 +4L \eta_{j,K,t}^2 \Gamma_{\text{cluster}} \nonumber\\
&\quad+ \eta_{j,K,t}^2 \sum_{K=1}^{M} q_K^{-1} \sum_{k\in \mathcal{S}_K} p_k^2 s_k^2 \nonumber\\
&\stackrel{(ii)}{\le} (1-\mu\eta_{j,K,t}) \mathbb{E} \|\overline{w}_{j,K,t}-W^*\|^2 + 4\eta_{j,K,t}^2 EMG^2 \nonumber\\
&\quad+ 1.5L\eta_{j,K,t}(4L)^{-1}(2\eta_{j,K,t})E^2G^2 \nonumber\\
&\quad+4L\eta_{j,K,t}^2 \Gamma_{\text{cluster}} + \eta_{j,K,t}^2 \sum_{K=1}^{M} q_K^{-1} \sum_{k\in \mathcal{S}_K} p_k^2 s_k^2 \nonumber\\
&\stackrel{(iii)}{\le} (1-\mu\eta_{j,K,t}) \mathbb{E} \|\overline{w}_{j,K,t}-W^*\|^2 + \eta_{j,K,t}^2 B \label{err_next_strongconvex}
\end{align}
where (i) uses \eqref{Gamma}, \eqref{eta_bound}, \eqref{SGvar_strongconvex}, \eqref{FedAvg_var_strongconvex}, \eqref{fromstar}, (ii) uses \eqref{eta_bound}, \eqref{jK0}, \eqref{j10} and (iii) uses the definition of $B$ in \eqref{B}.

By the update rule of \Cref{alg: 1}, $\overline{w}_{j,K+1,0}=\overline{w}_{j,K,E}=W_{jM+K+1}$ ($K=0,1,\ldots,M-2$) and $\overline{w}_{j+1,0,0}=\overline{w}_{j,M-1,E}=W_{(j+1)M}$. Hence, we can denote the total number of iterations up to iteration $t$ of cycle $K$ in round $j$ as {$s:=(jM+K)E+t$} and rewrite $\overline{w}_{j,K,t}:=\overline{w}_{(jM+K)E+t}=\overline{w}_{s}$, $\eta_{j,K,t}=\frac{2}{\mu[(jM+K)E+t+\gamma]}=\frac{2}{\mu(s+\gamma)}$. As a result, \eqref{err_next_strongconvex} can be rewritten as
\begin{align}\label{err_next_s}
\mathbb{E} \|\overline{w}_{s+1}-W^*\|^2 \le& \Big(1-\frac{2}{s+\gamma}\Big) \mathbb{E} \|\overline{w}_{s}-W^*\|^2 \nonumber\\
&+\frac{4B}{\mu^2(s+\gamma)^2}.
\end{align}
Telescoping \eqref{err_next_s} over $s$ and noting that $\overline{w}_{0}=\overline{w}_{0,0,0}=W_0$, we have
\begin{align}\label{L2err}
\mathbb{E} \|\overline{w}_{s}-W^*\|^2\le& \Big[\prod_{u=0}^{s-1} \Big(1-\frac{2}{u+\gamma}\Big) \Big] \mathbb{E}\|W_{0}-W^*\|^2 \nonumber\\
&+\sum_{v=0}^{s-1} \Big[\prod_{u=v+1}^{s-1} \Big(1-\frac{2}{u+\gamma}\Big)\Big] \frac{4B}{\mu^2(v+\gamma)^2} \nonumber\\
\stackrel{(i)}{\le}& \frac{(\gamma-2)(\gamma-1)}{(s+\gamma-2)(s+\gamma-1)} \mathbb{E}\|W_{0}-W^*\|^2 \nonumber\\
&+\sum_{v=0}^{s-1}\frac{(v+\gamma-1)(v+\gamma)}{(s+\gamma-2)(s+\gamma-1)} \frac{4B}{\mu^2(v+\gamma)^2}\nonumber\\
\le& \frac{(\gamma-2)(\gamma-1)}{(s+\gamma-2)(s+\gamma-1)} \mathbb{E}\|W_{0}-W^*\|^2 \nonumber\\
&+\frac{4sB}{\mu^2(s+\gamma-2)(s+\gamma-1)} \nonumber\\
\stackrel{(ii)}{\le}& \frac{\gamma G^2+4B}{\mu^2(s+\gamma-1)} \le \frac{\gamma G^2+4B}{\mu^2s},
\end{align}
\noindent where (i) uses the following \eqref{decay} (when $m=s$, both sides of \eqref{decay} equals 1), (ii) uses the facts that $\|W_{0}-W^*\|^2\le \mu^{-2}G^2$ {(since $f$ is $\mu$-strongly convex and that $\|\nabla f(W_0)\|\le G$ based on \eqref{fS_G})} and $0\le \frac{\gamma-2}{s+\gamma-2}, \frac{s}{s+\gamma-2}\le 1$ ($\gamma\ge \frac{8L}{\mu}\ge 8$). Finally, the desired result in \eqref{W_err_sc} follows from \eqref{L2err}, $W_{TM}=\overline{w}_{TME}$ and the $L$-smoothness of $f$.

\begin{align}\label{decay}
&\prod_{u=m}^{s-1} \Big(1-\frac{2}{u+\gamma}\Big)\nonumber\\
&=\prod_{u=m}^{s-1} \frac{(u+\gamma-2)(u+\gamma-1)}{(u+\gamma-1)(u+\gamma)}\nonumber\\
&= \frac{(m+\gamma-2)(m+\gamma-1)}{(s+\gamma-2)(s+\gamma-1)}, ~\text{where}~ 0\le m \le s.
\end{align}

Based on \eqref{W_err_sc}, a sufficient condition for $\mathbb{E}f(W_{TM}) - f(W^*) \le \epsilon$ is that
\begin{align}%\label{W_err_sc}
\frac{L(\gamma G^2 + 4B)}{2\mu^2TME}\le \epsilon, 
\end{align}
which implies that
\begin{align}\label{Teps_sc_derive}
	T\ge&  \frac{L(\gamma G^2 + 4B)}{2\mu^2\epsilon ME} \nonumber\\
	\stackrel{(i)}{=}&\mathcal{O} \Big[\frac{L(\gamma G^2 + B)}{\mu^2\epsilon ME}\Big]\nonumber\\
	\stackrel{(ii)}{=}&\mathcal{O} \Big\{\frac{L}{ME\mu^2\epsilon} \Big[ \Big(\frac{8L}{\mu}+ME\Big)G^2 + (EM+E^2)G^2\nonumber\\
	&\quad +L\Gamma_{\text{cluster}}+\sum_{K=1}^{M} q_K^{-1} \sum_{k\in \mathcal{S}_K} p_k^2 s_k^2 \Big]\Big\}\nonumber\\
	=&\mathcal{O}\Big\{\frac{L}{\mu^2\epsilon} \Big[\Big(1+\frac{E}{M}\Big)G^2+\frac{1}{EM}\Big(L\Gamma_{\textrm{cluster}}\nonumber\\ 
	&\quad+ \sum_{K=1}^{M} q_K^{-1} \sum_{k\in \mathcal{S}_K} p_k^2 s_k^2 + \frac{LG^2}{\mu}\Big) \Big]\Big\}\stackrel{\text{def}}{=} T_{\epsilon}
\end{align}
where (i) ignores the universal constants, (ii) uses $\gamma=\max\Big(\frac{8L}{\mu}, ME\Big)=\mathcal{O}(\frac{8L}{\mu}+ME)$ and  
\begin{align}
&B=\mathcal{O}\Big[(EM+E^2)G^2+L\Gamma_{\text{cluster}}+\sum_{K=1}^{M} q_K^{-1} \sum_{k\in \mathcal{S}_K} p_k^2 s_k^2\Big]\nonumber
\end{align}
as a result of \eqref{B}. Finally, \eqref{Teps_sc} follows from \eqref{Teps_sc_derive}. 
%
%\begin{align}%\label{Teps_sc}
%T_{\epsilon} \propto \frac{L}{\mu^2} \Big[\Big(1+\frac{E}{M}\Big)G^2+\frac{1}{EM}\Big(L\Gamma_{\textrm{cluster}} + \sum_{K=1}^{M} q_K^{-1} \sum_{k\in \mathcal{S}_K} p_k^2 s_k^2 + \frac{LG^2}{\mu}\Big) \Big].
%\end{align} 

%&B:=\Big(4EM+\frac{3}{4}E^2\Big)G^2+4L\Gamma_{\text{cluster}}+\sum_{K=1}^{M} q_K^{-1} \sum_{k\in \mathcal{S}_K} p_k^2 s_k^2 (to ~delete).\nonumber\\


==> thm_sc.tex <==
\subsection{Convergence Analysis in Strongly-Convex Optimization}
\vspace{-3pt}
In this subsection, we analyze the convergence rate of FedCluster with local SGD specified in \Cref{alg: 1} under strong-convexity of the loss function in the problem (P). 

Throughout the analysis of this paper, we define $q_K := \sum_{k\in \blue{S_k'}} p_k$ and $f(w; \mathcal{D}^{(\mathcal{S}_K)}) := q_K^{-1} \sum_{k\in \mathcal{S}_K} p_k f(w; \mathcal{D}^{(k)})$, which characterizes the total loss of the cluster $\mathcal{S}_K$. 
%Then, the total loss of the problem (P) can be alternatively written as $f(w) = \sum_{K=1}^M q_K f(w; \mathcal{D}^{(\mathcal{S}_K)})$. 
We also define $W^*:=\arg\min_{w\in\mathbb{R}^d} f(w)$, $f^*(\cdot;\mathcal{D}^{(\mathcal{S}_K)}):= \inf_{w\in\mathbb{R}^d} f(w;\mathcal{D}^{(\mathcal{S}_K)})$ and introduce the following notion of cluster-level data heterogeneity.
\begin{align}
&\Gamma_{\textrm{cluster}} := f(W^*) - \sum_{K=1}^{M} q_K f^*(\cdot;\mathcal{D}^{(\mathcal{S}_K)}).\label{Gamma} 
\end{align}
The above definition follows from the definition of device-level heterogeneity introduced in \cite{li2019convergence}. Intuitively, it measures the gap between the global minimum of total loss and that of the clusters' total loss. In particular, it vanishes when the clusters of devices have homogeneous datasets. 
We obtain the following convergence result of FedCluster.
\begin{thm}\label{thm: sc}
	Let \Cref{assum: P} hold and assume that $f(\cdot;\xi)$ is $\mu$-strongly convex for any data sample $\xi$. Choose learning rate {$\eta_{j,K,t} = \frac{2}{\mu [(jM +K)E+t+\gamma]}$}, where $\gamma=\max\Big(\frac{8L}{\mu}, ME\Big)$. \blue{Let every device participate in each round (i.e. $\mathcal{S}_{j, \sigma_j(K+1)}'\equiv \mathcal{S}_{\sigma_j(K+1)}$).} Then, the output of \Cref{alg: 1} satisfies
	\begin{align}\label{W_err_sc}
		\mathbb{E}f(W_{TM}) - f(W^*) &\le \frac{L(\gamma G^2 + 4B)}{2\mu^2TME}, 
	\end{align}
	where the constant $B$ is defined as	
	\begin{align}
		&B:=\Big(4EM+\frac{3}{4}E^2\Big)G^2+4L\Gamma_{\text{cluster}}+\sum_{K=1}^{M} q_K^{-1} \sum_{k\in \mathcal{S}_K} p_k^2 s_k^2\label{B}.
	\end{align}
	Furthermore, in order to achieve a solution that satisfies $\mathbb{E}f(W_{TM}) - f(W^*) \le \epsilon$, the required number of learning rounds $T$ satisfies
	\begin{align}\label{Teps_sc}
		T \propto& \frac{L}{\mu^2} \Big[\Big(1+\frac{E}{M}\Big)G^2+\frac{1}{EM}\Big(L\Gamma_{\textrm{cluster}}\nonumber\\
		 &+ \sum_{K=1}^{M} q_K^{-1} \sum_{k\in \mathcal{S}_K} p_k^2 s_k^2 + \frac{LG^2}{\mu}\Big) \Big].
	\end{align} 
\end{thm}

The above theorem shows that FedCluster with local SGD converges at a sublinear rate under strong convexity. Specifically, after $T$ learning rounds, the optimality gap of the total loss is in the order of \blue{$\mathcal{O}(\frac{1}{T}+\frac{E}{TM})$} \footnote{This rate incorporates $\mathcal{O}(EM+E^2)$ in $B$ defined by \eqref{B}.}. As a comparison, the FedAvg algorithm (i.e., conventional federated learning with local SGD) converges at the rate \blue{$\mathcal{O}(\frac{E}{T})$} \footnote{In \cite{li2019convergence}, $T$ is the total number of iterations, which equals to $TE$ in our setting where $T$ is the number of learning rounds. }, which is slower than FedCluster by a factor of \blue{$\min(M,E)\ge 1$}. Intuitively, this is \blue{partially} because FedCluster updates the global model $M$ times per learning round, whereas FedAvg updates it only once per learning round. On the other hand, note that the convergence rate of FedCluster is affected by the cluster-level data heterogeneity $\Gamma_{\textrm{cluster}}$ (see the definition of $B$ {in \eqref{B}}). As a comparison, the convergence rate of the FedAvg algorithm is affected by the device-level data heterogeneity $\Gamma_{\textrm{device}}:= f(W^*) - \sum_{k=1}^{n} p_k f^*(\cdot;\mathcal{D}^{(k)})$. In particular, it is easy to check that $\Gamma_{\textrm{cluster}}  \le \Gamma_{\textrm{device}}$, and therefore FedCluster suffers less from the data heterogeneity of the devices.  
Furthermore, in order to achieve an $\epsilon$ optimality gap, the FedAvg algorithm requires a total number of  learning rounds $T \propto \frac{L}{\mu^2} (EG^2+\frac{1}{E} (L\Gamma_{\textrm{device}} + \sum_{k=1}^{n} p_k^2 s_k^2 + \frac{LG^2}{\mu}))$ \footnote{The factor $\frac{L}{\mu^2}$ is missing in (8) of \cite{li2019convergence}.} In comparison, the number of learning rounds required by FedCluster in \eqref{Teps_sc} is only \blue{$\frac{1}{\min(E,M)}$} of that required by FedAvg and depends on the smaller cluster-level data heterogeneity. To summarize, FedCluster significantly boosts the convergence of the conventional federated learning via cluster cycling. 

The complexity result in \eqref{Teps_sc} implies the existence of an optimal choice of the number of local SGD iterations $E$, and hence one should tune a proper $E$ in practice. On the other hand, the term $\frac{\Gamma_{\text{cluster}}}{M}$ in \eqref{Teps_sc} also implies a trade-off between the number of clusters and the cluster-level data heterogeneity. Intuitively, having a large number of clusters $M$ will result in a large cluster-level data heterogeneity, and vice versa. Therefore, a proper choice of $M$ can benefit the overall performance. In our experiments, we found that FedCluster with multiple clusters ($M\ge 2$) always outperforms FedAvg. \blue{For a given $M$, a  clustering choice with smaller cluster-level data heterogeneity $\Gamma_{\text{cluster}}$ has a faster convergece rate.}

The proof of \Cref{thm: sc} requires substantial new developments to address the following unique challenges in analyzing FedCluster with local SGD.  First, each learning round of FedCluster with local SGD consists of $M$ inner cycles, and each cycle activates only one cluster to perform federated learning via the FedAvg algorithm. In our analysis, we track the model average $\overline{w}_{j,K,t}$ of the local models of the current active cluster $\mathcal{S}_{\sigma_{j}(K+1)}$ and estimate the per-iteration optimization progress of the local updates in terms of the distance-to-minimizer $\|\overline{w}_{j,K,t}-W^*\|^2$.
Second, the cluster activation order $\sigma_j(K+1), K=0,...,M-1$ is generated by random reshuffling and hence are {\em dependent} from each other, which also causes the dependency among the data samples $\xi_{j,K,t}^{(k)}$ sampled by the devices of different clusters in different cycles. In our analysis of the inner cycles of the $j$-th round, we propose to use the reference point  $W_{jM}$ that is independent of all the randomness of the $j$-th round to help estimate the error bounds in \Cref{lemma_FedAvg_howfar_strongconvex,lemma_fromstar}.

